Impacts of high-contrast image processing on atmospheric retrievals

Many post-processing algorithms have been developed in order to better separate the signal of a companion from the bright light of the host star, but the effect of such algorithms on the shape of exoplanet spectra extracted from integral field spectrograph data is poorly understood. The resulting spectra are affected by noise that is correlated in wavelength space due to both optical and data processing effects. Within the framework of Bayesian atmospheric retrievals, we aim to understand how these correlations and other systematic effects impact the inferred physical parameters. We consider three algorithms (KLIP, PynPoint and ANDROMEDA), optimizing the choice of algorithmic parameters using a series of injection tests into archival SPHERE and GPI data of the HR 8799 system. The wavelength-dependent covariance matrix is calculated to provide a measure of instrumental and algorithmic systematics. We perform atmospheric retrievals using petitRADTRANS on optimally extracted spectra to measure how these data processing systematics influence the retrieved parameter distributions. The choice of data processing algorithm and parameters significantly impact the accuracy of retrieval results, with the mean posterior parameter bias ranging from 1 to 3 $\sigma$ from the true input parameters. Including the full covariance matrix in the likelihood improves the accuracy of inferred parameters, and cannot be accounted for using ad hoc scaling parameters in the retrieval framework. Using the Bayesian information criterion and other statistical measures as a heuristic goodness-of-fit metrics, the retrievals including the full covariance matrix are favoured when compared to using only the diagonal elements.

==> DirectImagingRetrievalSystematics/commands.tex <==

\def\ptrad{{\tt petitRADTRANS}\xspace}
\def\klip{{\tt KLIP}\xspace}

\def\ptdoc{\url{https://petitradtrans.readthedocs.io}}

\def\mearth{{\rm M}_\oplus}
\def\rearth{{\rm R}_\oplus}
\def\ed{{\sc{EddySed}}\xspace}

\def\msun{{\rm M}_\odot}
\def\rsun{{\rm R}_\odot}
\def\rhill{R_{\rm H}}
\def\mcore{M_{\rm core}}
\def\mheavy{M_{\rm heavy}}
\def\astart{a_{\rm start}}
\def\fpg{f_{\rm D/G}} 
\def\fri{f_{\rm R/I}}
\def\f1{f_{\rm I}}
\def\mj{{\rm M}_{\textrm{\tiny \jupiter }}}
\newcommand{\lj}{{\rm L}_{\textrm{\tiny \jupiter}}}
\newcommand{\rj}{{\rm R}_{\textrm{\tiny \jupiter}}}
\newcommand{\pyklip}{{\tt pyKLIP}\xspace}
\newcommand{\pyn}{{\tt Pynpoint}\xspace}
\def\teff{$T_{\rm eff}$}
\def\kzz{$K_{zz}$\xspace}
\def\fsed{$f_{sed}$\xspace}
\def\h2o{H$_{2}$O\xspace}
\def\ch4{CH$_{4}$\xspace}
\def\nh3{NH$_{3}$\xspace}
\def\co2{CO$_{2}$\xspace}
\def\ph3{PH$_{3}$\xspace}


\def\mstar{M_*}
\def\mdisk{M_{\rm disk}}
\def\astart{a_{\rm start}}
\def\tstart{t_{\rm start}}
\def\membstart{M_{\rm emb,0}}
\def\memb{M_{\rm emb}}
\def\anorm{a_0}
\def\rcore{R_{\rm core}}
\def\mdotcore{\dot{M}_{\rm core}}
\def\mwind{\dot{M}_{\rm w}}
\def\menv{M_{\rm env}}
\def\miso{M_{\rm iso}}
\def\mpla{m_{\rm pla}}
\def\arock{a_{\rm rock}}
\def\aice{a_{\rm ice}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\mplanet{M_{\rm planet}}
\def\aplanet{a_{\rm planet}}
\def\sigmad{\Sigma_{\rm D}}
\def\atouch{a_{\rm touch}}
\def\sigmanorm{\Sigma_{0}}
\def\tmc{\tau_{\rm RV,MC}}
\def\epsilonmc{\epsilon_{\rm RV,MC}}
\def\nref{N_{\rm ref}}
\def\nobsref{N_{\rm obsref}}
\def\nhot{N_{\rm hot}}
\def\nlate{N_{\rm late}}
\def\nobs{N_{\rm obs}}
\def\nsamp{N_{\rm samp}}
\def\dks{d_{\rm KS}}
\def\sam{S_{\rm a-M}}
\def\sm{S_{\rm M}}
\def\sa{S_{\rm a}}
\def\sfeh{S_{\rm [Fe/H]}}
\def\nobsreffv{N_{\rm obsrefFV}}
\def\nobsrefhotfv{N_{\rm obsrefhotFV}}
\def\msini{M\sin i}
\def\amax{a_{\rm max}}
\def\amin{a_{\rm min}}
\def\aphys{a_{\rm phys}}
\def\pwhot{P_{\rm whot}}
\def\pfv{P_{\rm FV}}
\def\pfvwhot{P_{\rm FV,whot}}
\def\ffv{F_{\rm FV}}
\def\fwemb{F_{\rm wemb}}
\def\mmax{M_{\rm max}}

\def\fopa{f_{\rm opa}}
\def\t2{\tau_{\rm II}}
\def\ltot{L_{\rm tot}}
\def\lcore{L_{\rm core}}
\def\mtot{M_{\rm tot}}
\def\sigmas0{\Sigma_{\rm s,0}}
\def\LJ{L_{{\rm \jupiter}}}
\def\RJ{R_{{\rm \jupiter}}}

\def\petit{\emph{petitCODE}\ }


\newcommand{\kgold}{K_{\rm Gold}}
\newcommand{\kliss}{K_{\rm Liss}}
\newcommand{\bliss}{B_{\rm Liss}}
\newcommand{\rcapt}{R_{\rm capt}}
\newcommand{\mz}{M_{\rm Z}}
\newcommand{\mxy}{M_{\rm XY}}
\newcommand{\lext}{L_{\rm ext}}
\newcommand{\lsun}{L_{\odot}}
%\newcommand{\astart}{a_{\rm start}}
\newcommand{\fpgsun}{f_{\rm D/G,\odot}} 
%\newcommand{\f1}{f_{\rm I}}

\newcommand{\mdisc}{M_{\rm disc}}
\newcommand{\tdisc}{t_{\rm disc}}
\newcommand{\mdotz}{\dot{M}_{\rm Z}}
\newcommand{\mdotxy}{\dot{M}_{\rm XY}}

\newcommand{\cadia}{C_{\rm adia }}
\newcommand{\cloc}{C_{\rm loc }}
\newcommand{\fvisc}{f_{\rm visc }}
\newcommand{\fsigma}{f_{\rm \Sigma}}
\newcommand{\xs}{x_{\rm s}}
\newcommand{\rp}{r_{\rm p}}
\newcommand{\omegap}{\Omega_{\rm p}}
\newcommand{\sigmap}{\Sigma_{\rm p}}
\newcommand{\tauuturn}{\tau_{\rm U-turn}}
\newcommand{\taucool}{\tau_{\rm cool}}
\newcommand{\taulib}{\tau_{\rm lib}}
\newcommand{\tauvisc}{\tau_{\rm visc}}
\newcommand{\msat}{M_{\rm sat}}
\newcommand{\mgap}{M_{\rm gap}}
\newcommand{\rroche}{r_{\rm Roche}}
\newcommand{\betat}{\beta_{\rm T}}
\newcommand{\betas}{\beta_{\rm \Sigma}}
\newcommand{\dotrp}{\dot{r}_{\rm p}}


\makeatletter
\let\jnl@style=\rm
\def\ref@jnl#1{{\jnl@style#1}}

\def\aj{\ref@jnl{AJ}}                   % Astronomical Journal
\def\actaa{\ref@jnl{Acta Astron.}}      % Acta Astronomica
\def\araa{\ref@jnl{ARA\&A}}             % Annual Review of Astron and Astrophys
\def\apj{\ref@jnl{ApJ}}                 % Astrophysical Journal
\def\apjl{\ref@jnl{ApJ}}                % Astrophysical Journal, Letters
\def\apjs{\ref@jnl{ApJS}}               % Astrophysical Journal, Supplement
\def\ao{\ref@jnl{Appl.~Opt.}}           % Applied Optics
\def\apss{\ref@jnl{Ap\&SS}}             % Astrophysics and Space Science
\def\aap{\ref@jnl{A\&A}}                % Astronomy and Astrophysics
\def\aapr{\ref@jnl{A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\def\aaps{\ref@jnl{A\&AS}}              % Astronomy and Astrophysics, Supplement
\def\azh{\ref@jnl{AZh}}                 % Astronomicheskii Zhurnal
\def\baas{\ref@jnl{BAAS}}               % Bulletin of the AAS
\def\bac{\ref@jnl{Bull. astr. Inst. Czechosl.}}
                % Bulletin of the Astronomical Institutes of Czechoslovakia 
\def\caa{\ref@jnl{Chinese Astron. Astrophys.}}
                % Chinese Astronomy and Astrophysics
\def\cjaa{\ref@jnl{Chinese J. Astron. Astrophys.}}
                % Chinese Journal of Astronomy and Astrophysics
\def\icarus{\ref@jnl{Icarus}}           % Icarus
\def\jcap{\ref@jnl{J. Cosmology Astropart. Phys.}}
                % Journal of Cosmology and Astroparticle Physicshttps://www.overleaf.com/project/639113f4df4bea6928ff58cb
\def\jrasc{\ref@jnl{JRASC}}             % Journal of the RAS of Canada
\def\memras{\ref@jnl{MmRAS}}            % Memoirs of the RAS
\def\mnras{\ref@jnl{MNRAS}}             % Monthly Notices of the RAS
\def\na{\ref@jnl{New A}}                % New Astronomy
\def\nar{\ref@jnl{New A Rev.}}          % New Astronomy Review
\def\pra{\ref@jnl{Phys.~Rev.~A}}        % Physical Review A: General Physics
\def\prb{\ref@jnl{Phys.~Rev.~B}}        % Physical Review B: Solid State
\def\prc{\ref@jnl{Phys.~Rev.~C}}        % Physical Review C
\def\prd{\ref@jnl{Phys.~Rev.~D}}        % Physical Review D
\def\pre{\ref@jnl{Phys.~Rev.~E}}        % Physical Review E
\def\prl{\ref@jnl{Phys.~Rev.~Lett.}}    % Physical Review Letters
\def\pasa{\ref@jnl{PASA}}               % Publications of the Astron. Soc. of Australia
\def\pasp{\ref@jnl{PASP}}               % Publications of the ASP
\def\pasj{\ref@jnl{PASJ}}               % Publications of the ASJ
\def\rmxaa{\ref@jnl{Rev. Mexicana Astron. Astrofis.}}%
                % Revista Mexicana de Astronomia y Astrofisica
\def\qjras{\ref@jnl{QJRAS}}             % Quarterly Journal of the RAS
\def\skytel{\ref@jnl{S\&T}}             % Sky and Telescope
\def\solphys{\ref@jnl{Sol.~Phys.}}      % Solar Physics
\def\sovast{\ref@jnl{Soviet~Ast.}}      % Soviet Astronomy
\def\ssr{\ref@jnl{Space~Sci.~Rev.}}     % Space Science Reviews
\def\zap{\ref@jnl{ZAp}}                 % Zeitschrift fuer Astrophysik
\def\nat{\ref@jnl{Nature}}              % Nature
\def\iaucirc{\ref@jnl{IAU~Circ.}}       % IAU Cirulars
\def\aplett{\ref@jnl{Astrophys.~Lett.}} % Astrophysics Letters
\def\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}
                % Astrophysics Space Physics Research
\def\bain{\ref@jnl{Bull.~Astron.~Inst.~Netherlands}} 
                % Bulletin Astronomical Institute of the Netherlands
\def\fcp{\ref@jnl{Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\def\gca{\ref@jnl{Geochim.~Cosmochim.~Acta}}   % Geochimica Cosmochimica Acta
\def\grl{\ref@jnl{Geophys.~Res.~Lett.}} % Geophysics Research Letters
\def\jcp{\ref@jnl{J.~Chem.~Phys.}}      % Journal of Chemical Physics
\def\jgr{\ref@jnl{J.~Geophys.~Res.}}    % Journal of Geophysics Research
\def\jqsrt{\ref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\def\memsai{\ref@jnl{Mem.~Soc.~Astron.~Italiana}}
                % Mem. Societa Astronomica Italiana
\def\nphysa{\ref@jnl{Nucl.~Phys.~A}}   % Nuclear Physics A
\def\physrep{\ref@jnl{Phys.~Rep.}}   % Physics Reports
\def\physscr{\ref@jnl{Phys.~Scr}}   % Physica Scripta
\def\planss{\ref@jnl{Planet.~Space~Sci.}}   % Planetary Space Science
\def\procspie{\ref@jnl{Proc.~SPIE}}   % Proceedings of the SPIE

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
\makeatother

\def\ptp{\ref@jnl{Prog.~Th.~Phys.}}   % Progress of Theoretical Physics

\def\vol#1{ #1}
\def\({\left(}
\def\){\right)}
\def\<{\left<}
\def\>{\right>}

\def\bacon{\emph{BACON}~}
\def\tr{\mathcal{T}}

\newcommand{\rch}[1]{{{\color{orange}#1}}}
\newcommand{\rea}[1]{{{\color{red}Reading: #1}}}
%\newcommand{\cstart}{{\textbf{\color{green}CHECK START}}}
%\newcommand{\cend}{{\textbf{\color{green}CHECK END}}}
\newcommand{\cstart}{}
\newcommand{\cend}{}

